An Explicit Skew-Hadamard Matrix of Order 1252 via Cyclotomic Unions

We construct a skew-Hadamard matrix of order 1252 = 2(5^4 + 1) using a bordered skew-Hadamard difference family over GF(5^4), with blocks given as unions of cyclotomic classes of order N = 16. This order has been reported as missing in some widely used open-source computational tables; we provide an explicit instance together with verification artifacts. We prove the structural prerequisites for the bordered construction (skew-symmetry of one block and the constant autocorrelation-sum condition), and we compute algebraic invariants to facilitate classification: the associated tournament adjacency matrix has full rank over GF(2), and the matrix has full rank over GF(3) and GF(5). We also exhibit an explicit affine subgroup of the automorphism group of size 24 375. All claims are supported by a reproducible artifact bundle including the explicit matrix and verification logs.

==> hash_table_1252.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lp{9cm}}
\toprule
Filename & SHA-256 Hash \\
\midrule
blocks\_1252.json & \texttt{bc3b5d940eb58ebcb022b520bc2af43ccb2f18823ab29691a634991c812f5253} \\
matrix\_1252.txt & \texttt{feb0eaa5d7f8f1862ff67e3acc681579763eaad74c1e4da9435ae447c0c9d78a} \\
verify\_sage.py & \texttt{ed2dad54e84a101aceb51a21b5175d9b0569bc5f7cc74611812560ab20690de8} \\
\bottomrule
\end{tabular}
\caption{Cryptographic hashes of immutable core artifacts (manifest\_core.json).}
\label{tab:hashes}
\end{table}
